Hyper-Spectral Image Analysis with Partially-Latent Regression and Spatial Markov Dependencies

Hyper-spectral data can be analyzed to recover physical properties at large planetary scales. This involves resolving inverse problems which can be addressed within machine learning, with the advantage that, once a relationship between physical parameters and spectra has been established in a data-driven fashion, the learned relationship can be used to estimate physical parameters for new hyper-spectral observations. Within this framework, we propose a spatially-constrained and partially-latent regression method which maps high-dimensional inputs (hyper-spectral images) onto low-dimensional responses (physical parameters such as the local chemical composition of the soil). The proposed regression model comprises two key features. Firstly, it combines a Gaussian mixture of locally-linear mappings (GLLiM) with a partially-latent response model. While the former makes high-dimensional regression tractable, the latter enables to deal with physical parameters that cannot be observed or, more generally, with data contaminated by experimental artifacts that cannot be explained with noise models. Secondly, spatial constraints are introduced in the model through a Markov random field (MRF) prior which provides a spatial structure to the Gaussian-mixture hidden variables. Experiments conducted on a database composed of remotely sensed observations collected from the Mars planet by the Mars Express orbiter demonstrate the effectiveness of the proposed model.

==> CoverLetter-R1.tex <==
\begin{coverletter}{Hyper-Spectral Image Analysis with Partially-Latent\\ Regression and Spatial Markov Dependencies}{J-STSP-AHDPA-00230-2014}

\begin{answereditor}{Based on the enclosed set of reviews, I am recommending that the manuscript undergo MAJOR REVISONS (RQ)}
The submission was reviewed by two reviewers. They both recommend \textbf{major} revisions. The authors would like to warmly thank the reviewers for their dedicated reviews with serious and highly valuable comments and suggestions. The authors prepared a revised version of the manuscript. \textbf{An annotated version of this new manuscript with modifications highlighted in green and numbered C1, C2, etc., is attached at the end of this pdf. The authors' replies in the cover letter refer to these annotations, e.g., C4 on P4, means that annotation C4 can be found on page 4}. 

The main revisions are the followings:
\begin{enumerate}
\item We completely revised section III to make our theoretical contribution clearer. At the end of this section we added a short overview of both the learning and prediction procedures proposed in the paper.   A pseudocode describing the main steps of the MRF-GLLiM model was added in Section III-D.
\item We made several additions to the manuscript, namely in the abstract, introduction and experimental section to explain more explicitly what is meant by physical parameters, namely \refcm{physical1}, \refcm{physical2}, \refcm{physical3} and \refcm{physical4}.
%\item In Section III-D a pseudocode describing the main steps of the MRF-GLLiM model is given in order to ease understanding.
\item Section III-B was re-written in order to clarify that a gradient descent procedure was used to estimate the MRF prior distribution parameters.
\item We added a new Section IV-B in which synthetic data are generated and processed. In this new section, the Markov random field prior parameters of the MRF-GLLiM are estimated using gradient descent as described in Section III-B. Furthermore, GLLiM and MRF-GLLiM numerical performance comparison provided in Table~\ref{tab:planeto_spatial_err} demonstrates the effectiveness of the latter model. 
\end{enumerate}
\end{answereditor}

%answers to the first reviewer
\begin{answerreviewer}[\textit{Recommendation: RQ - Review Again After Major Changes}. \newline
The paper presents a method for the analysis of hyper-spectral images. The aim of the paper is to find relationships between hyper-spectral images and physical properties of the area of interest. The proposed method introduces spatial constraints through a Markov Random Field in a recently proposed model (Ref \cite{DeleforgeForbesHoraud2014}) based on the Gaussian mixture of locally-linear mapping in order to have smoother solutions.\\ \newline
The paper is well motivated and the presentation of the state of the art is clear and quite complete in the Introduction. Unfortunately, I found the paper somewhat ambiguous and sometimes difficult to read in the successive sections mainly for two reasons: i) section III is dense of formulas and the actual role of the proposed refinement in the general model and its embedding in the existing method seem masked; ii) there is ambiguity between the proposed method and the one in Ref \cite{DeleforgeForbesHoraud2014}, especially in the section of experimental results. ]

\qa{With regard to the first point, a pseudocode or a block scheme of the proposed procedure would help the immediate understanding of the whole procedure and the role of each step, including the proposed refinement. This would also make the paper self-contained. In addition, not all the equations in Section III are essential in a general reading of the paper. I suggest to rearrange this section in order to leave just the main concepts and formulas necessary to understand the proposed refinement, how MRF constraint is used and where and in what way it is embedded in the model in Ref \cite{DeleforgeForbesHoraud2014}. The other details should be moved in the Appendix for interested readers. 
}
{We completely reorganized section~\ref{sec:variational-EM} with additional explanations (\refcm{revision11}). We followed the advice of the reviewer and added a subsection (III.D) that overviews the proposed method (\refcm{outline}). This section is the main theoretical contribution of the paper and our position is that it should be self contained.}

\qa{With regard to the second point, in the section IV MRF-hGLLiM results (that is the proposed method, as stated in the preceding sections and in Section IV.A) have been presented just for real images (Section IV.C). For synthetic data, only the results for the hybrid model (hGLLiM) with a different number of latent variables have been presented. The authors should better clarify this point. If the novelty of the paper is the introduction of MRF spatial constraint, its contribution and benefits should be showed also for synthetic data. By setting the parameter beta equal to zero, MRF-hGLLiM is equivalent to the existing method in  \cite{DeleforgeForbesHoraud2014}. A direct comparison with  \cite{DeleforgeForbesHoraud2014} should be introduced since table 1: what is the advantage in using the proposed method in terms of accuracy of the results and computing time (with and without BIC)? 
}
{The reviewer rightfully points out that the previous version of our manuscript did not include quantitative results on synthetic hyper-spectral images. For this updated version, we developed a procedure for generating synthetic hyper-spectral images and ran new experiments on them. This yielded a new experimental section, namely section \ref{sec:synth_images}, \refcm{synth_images}, composed of two paragraph, \refcm{numeval1} and \refcm{numeval2}. As asked by the reviewer, this section includes a quantitative comparison between hGLLiM with and without MRF prior on these synthetic images (Table \ref{tab:planeto_spatial_err}). These new results show the benefits of the proposed MRF framework.}

\qa{Furthermore, beta is a parameter that has to be fixed a priori and it fixes the regularity of the data. Some discussions about how it can be selected (in an automatic or guided way) should be included in Section IV. Is there a criterion for selecting it in an adaptive manner? In this sense the proposed model seems to have similar drawbacks of the works in Refs [17],[22-24] that cannot select the kernel function in an automatic way. In addition, the selection of the expected latent variables should be discussed more in depth. Some discussions and comments about the convenience in using BIC instead of selecting Lw in an arbitrary way should be included in Section IV. }
{Although the full variational EM procedure, including estimation of $\beta$, was provided in the previous manuscript, we had not provided numerical details on how to solve its estimation, and we had not tested the automatic estimation of $\beta$ in the experimental section. Following the reviewer's remark, we addressed both these issues in the new version of the manuscript. Section \ref{subsec:variational} (\refcm{vmstep}) was completely re-written to provide details on the gradient descent method used to estimate $\beta$. Moreover, the new experimental section \ref{subsection:synth_images} presents results obtained by automatically estimating $\beta$ using synthetic images. A detailed experimental analysis on the advantage of using BIC with respect to arbitrary values of $L_{\textrm{w}}$ is provided in Table~\ref{tab:planeto_err} and associated discussions in \refcm{bic}.}
\end{answerreviewer}

%answers to the second reviewer
\begin{answerreviewer}[\textit{Recommendation: RQ - Review Again After Major Changes}. \newline
This work first combines a Gaussian mixture of locally linear mappings with a partially latent response model, and then introduces a spatial constrained MRF prior. This reviewer has some comments which are list in the following. 
]

\qa{The proposed approach is very interesting, while its application to the Mars data is also very professional. The comment is that, is the proposed approach specified for Mars data? Or is it suitable for any hyperspectral data? If it works with all hyperspectral data, a recommendation is to validate the proposed approach with some other data, such as data from the earth. 
}
{Thank you for these questions. The proposed approach is in principle suitable for any hyper-spectral data. Unfortunately, we could not access a dataset of Earth images that is \textit{(i)} sufficiently large to learn the model parameters, \textit{(ii)} presents a non-linear relationship between spectra and physical parameters and \textit{(iii)} features spatial dependencies between spectra. We therefore focused on the Mars image dataset presented in the manuscript. A paragraph justifying this choice in details has been added in \refcm{otherdata}.}

\qa{In the manuscript, authors stated that `...which maps high-dimensional inputs (hyper-spectral images) onto low-dimensional responses (physical parameters...' what do physical parameters mean? What is the exact definition? Please give quantitative and qualitative analysis with respect to this aspect in the experimental sections. }
{We made several additions to the manuscript, namely in the abstract, introduction and experimental section to explain more explicitly what is meant by physical parameters, namely \refcm{physical1}, \refcm{physical2}, \refcm{physical3} and \refcm{physical4}. In the case of the Mars dataset, the physical parameters are 
the proportion of water, the proportion of CO$_2$ ice, the proportion of dust, the grain size of water ice and the grain size of CO$_2$ ice.
}

\qa{Computational complexity should be discussed.}
{Following the reviewer's remark, we added three notes on computational complexity, namely \refcm{complexity1a}, \refcm{complexity1b} and \refcm{complexity2}.}

\qa{In the literature, there are many studies, which map the high dimensional hyperspectral data to low dimensional subspaces, and then use MRF spatial regularizer. Authors are recommended to make a better review. For instance: 

\cite{Li2012} J. Li, J. Bioucas-Dias and A. Plaza. Spectral-Spatial Hyperspectral Image Segmentation Using Subspace Multinomial Logistic Regression and Markov Random Fields. IEEE Transactions on Geoscience and Remote Sensing, vol. 50, no. 3, pp. 809-823, 2012. }
{Indeed, the dimension of the space spanned by spectra from an image is generally much lower than the available number of bands. When the goal is to characterize observed spectra with a limited number of features (such as abundances or physical characteristics), identifying appropriate subspaces can then improve performance significantly. In general, such dimension reduction aims at representing spatial vectors in a lower more tractable space in which noise can be better characterized.  This reduction step is then often an intermediate step before additional refinement such as the inclusion of contextual information is performed. In \cite{Li2012}, dimension reduction and Markov modeling are carried out in two successive steps and assuming a linear mixing model. This is quite different from our approach which aims at modeling and identifying non-linear mappings and not necessarily in the unmixing context only.  In our work,  the high-to-low mapping is a target  while it is only a convenient intermediate step in most studies. Also, in our approach, the Markov field is  directly included in the generative modeling of the high-to-low dimensional mapping. 
Of course, considering the high level of activity in hyperspectral image analysis, it is challenging to present an exhaustive view of the subject but we believe that methods using subspace reduction in this field correspond to a different use of dimensionality reduction. We refer to \cite{Bioucas-Dias2012} for one recent review on both subspace identification and spatial modeling. We added this comment in the manuscript \refcm{addbiblio}. 

\cite{Bioucas-Dias2012} J. Boucias-Dias, A. Plaza, N. Dobigeon, M. Parente, Q. Du, P. Gader, J. Chanussot. Hyperspectral unmixing overview: Geometrical, statistical and sparse regression-based approaches. IEEE journal of selected topics in applied earth observations and remote sensing, Vol. 5, No 2. April 2012.

}


\end{answerreviewer}

\end{coverletter}

